Anonymized Local Privacy

In this paper, we introduce the family of Anonymized Local Privacy mechanisms. These mechanisms have an output space of three values "Yes", "No", or "$\perp$" (not participating) and leverage the law of large numbers to generate linear noise in the number of data owners to protect privacy both before and after aggregation yet preserve accuracy. We describe the suitability in a distributed on-demand network and evaluate over a real dataset as we scale the population.

==> evaluation.tex <==
\section{Evaluation}

\begin{figure*}[ht!]
    \includegraphics[width=1\textwidth]{figs/estimation}
    \caption{\textbf{Accuracy.} Ground truth versus privatized vehicle counts with a 99\% confidence interval. The population not at the station being monitored (i.e., $No$ population) is increases by expanding the query to the population listed in the table.}
        \label{fig:trafficdata}
\end{figure*}

\subsection{Accuracy}
\label{sec:evaluation:accuracy}

We evaluate the Anonymized Local Privacy optimal mechanism over a real dataset rather than arbitrary distributions. We utilize the California Transportation Dataset from magnetic pavement sensors~\cite{pems} collected in LA$\backslash$Ventura California freeways~\cite{cwwpinformation}.  There are a total of 3,220 stations and 47,719 vehicles total. We assign virtual identities to each vehicle. Each vehicle announces the station it is currently at.

Figure~\ref{fig:trafficdata} compares the Anonymized Local Privacy mechanism to the ground truth data over a 24 hour time period with a confidence interval of 99\%. We select a single popular highway station that collects and aggregates vehicle counts every 30 seconds. (For reasons of illustration we graph a subset of points for readability). We assign virtual identifiers and have every vehicle at the monitored station truthfully report ``Yes" while every other vehicle in the population truthfully reports ``No". The Anonymized Local Privacy mechanism then privatizes each vehicle's response. Traffic management analyzing the privatized time series would be able to infer the ebbs and flow of the vehicular traffic. 

The coin toss probabilities are fixed and the sampling $No$ rate is adjusted for privacy and error guarantees. The parameters $\pi_{s_{Yes_{1}}}=0.45$, $\pi_{s_{Yes_{2}}}=0.50$,  $\pi_1=0.95$, $\pi_2=0.98$, $\pi_3=0.98$ are fixed and $\pi_{s_{No}}=0.068$ varies from $0.068$ to $0.00000068$.

\subsection{Privacy}
\label{sec:evaluation:privacy}

We evaluate privacy strength of the Anonymized Local Privacy mechanism by examining the crowd sizes. We use the binomial complementary cumulative distribution function (ccdf) to determine the threshold of the number of successes. The crowd blending size is controlled by the $No$ population, that is the number of data owners that truthfully respond ``No". Also, the data owner blends in the $\perp$ crowd, that is the crowd which is not participating.

%Aggressive sampling ensures that less than 5\% of the $Yes$ population responds with a truthful ``Yes" and a similar percentage responds ``Yes" with plausible deniability (controlled by  $\pi_{s_{Yes_{1}}}$ and  $\pi_{s_{Yes_{2}}}$).

The number of crowds an single owner blends is determined by the number of queries (e.g., number of crowdsourced locations). The coin toss probability of  ($\pi_{s_{No}} \times \pi_3$) magnifies the number of crowds, that is the number of queries that the data owner will respond to. Also, the data owner blends in the $\perp$ crowd.

Table~\ref{tab:locations} shows the number of additional locations a single data owner will respond to out of 3,320. Decreasing the sampling rate causes a reduction in the number of additional locations. In this case, the mechanism essentially ignores the data owner as the aggregate output information is essentially the same output distribution as show by the graph. As each data owner reports they are at their actual location less than 5\% of the time, the additional three simultaneous announcements provides adequate privacy protection.

Table~\ref{tab:dataowners} shows the number of data owners an individual will blend with. We vary the population of additional data owners and accordingly decrease the sampling rate $\pi_{No}$ to calibrate the error. The noise added is linear with the number of data owners to protect. Sampling reduces the the crowd size yet at the same time provides privacy protection.

\begin{table}[]
%\small
\Huge
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l}
\textbf{Locations} & \textbf{TossThree($\pi_3$)} & \textbf{SamplingRate($\pi_{s_{No}}$)} & \textbf{Number Stations} \\ \hline
1                & 0.98              & 0.05  & 3320        \\ \hline
3                & 0.98             & 0.00025   & 83,000        \\ \hline              
3                & 0.98             & 0.000025   & 830,000        \\ \hline                          
\end{tabular}%
}
\caption{\textbf{Multiple Locations.} A single data owner will claim to be in multiple locations simultaneously.}
\label{tab:locations}
\end{table}

\begin{table}[]
%\small
\Huge
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l}
\textbf{CrowdSize} & \textbf{TossThree($\pi_3$)} & \textbf{SamplingRate($\pi_{s_{No}}$)} & \textbf{Population} \\ \hline
160                   & 0.98              & 0.05       &  48,719           \\ \hline
140                  & 0.98             & 0.00025        & 1,047,719            \\ \hline
130                  & 0.98             & 0.000025        & 10,047,719            \\ \hline           
\end{tabular}%
}
\caption{\textbf{Crowd size.} A single data owner blends with $k$ other data owners who noisily answer ``Yes" from the $No$ population .}
\label{tab:dataowners}
\end{table}



%~\\
%\noindent \textbf{Crowd Size.}

%~\\
%\noindent \textbf{Multiple Crowds.}

==> goals.tex <==
\section{Goals and Problem Statement}

We describe the system model, system goals, performance goals, and threat model of the Anonymized Local Privacy mechanism. 

\input{systemmodel}

\subsection{System Goals}

We now define the query model and response.

%The goals for our system as follows. The protocol does not require a restart if a mobile node (e.g., smartphone or vehicle) enters or leaves. Messages received are processed in the same epoch in which they are received, regardless of whether they are at the beginning or end of the epoch.

%In addition, the analysts are deemed to be reputable, e.g., Department of Transportation, National Institutes of Health, or Centers for Disease Control. Each analyst may own or contribute an aggregation server.  Aggregation servers may also be contributed by privacy watchdog groups such as the Electronic Frontier Foundation (EFF). \\

%The system should support analysts who wish to learn statistics about the population. The analysts issue a statistical query and then all data owners locally privatize their data and privately write their reply. The queries are fetched only once by each data owner. Data owners have the choice of answering or not answering the query and can configure their devices to respond only if certain conditions are met (e.g., whitelisting or blacklisting certain sensors or response frequency).

\input{query}



==> privacy.tex <==
\section{Privacy Guarantee}

\subsection{Differential Privacy Guarantee}

Anonymized Local Privacy satisfies differential privacy. We utilize the same proof structure as shown by Claim 3.5 in~\cite{DBLP:journals/fttcs/DworkR14}. Let ``Yes'' be the privatized response and $Yes$ and $No$ be the respective populations.

\begin{equation}
\epsilon_{DP} = \max \Bigg({\ln \bigg(\frac{\Pr[\textrm{``Yes" \textbar $Yes$}]} {\Pr[\textrm{``Yes" \textbar $No$}]} \bigg),\ln \bigg(\frac{\Pr[\textrm{``No" \textbar $No$}]} {\Pr[\textrm{``No" \textbar $Yes$}]} \bigg)} \Bigg)
\end{equation}

\begin{equation}
\epsilon_1 = \ln \Bigg( \frac{ \pi_{s_{Yes_{1}}} \times \pi_1 + \pi_{s_{Yes_{2}}} \times \pi_2 }{ \pi_{s_{No}} \times \pi_3 } \Bigg)
\end{equation}

\begin{equation}
\epsilon_2 = \ln \Bigg( \frac{ \pi_{s_{No}} \times (1-\pi_3) }{ \pi_{s_{Yes_{1}}} \times (1 - \pi_1) + \pi_{s_{Yes_{2}}} \times (1 - \pi_2) } \Bigg)
\end{equation}

\begin{equation}
\epsilon_{DP} = \max(\epsilon_1,\epsilon_2) 
\end{equation}




==> query.tex <==

~ \\
\noindent \textbf{Query Formulation.} An example query may be ``what is the distribution of vehicles across the New York City metro area?". Here, the analyst can define $L$ indexes corresponding to locations: `Statue of LIberty', `Empire State Building', $\cdots$,  `Brooklyn Bridge'.  If a vehicle is currently at the Statue of Liberty, the data owner on that vehicle truthfully answers `1' for the first index, and `0' for all others. In Section ~\S\ref{sec:optimalmechanism} we explain how we privatize the response.


Thus, each query specifies a few fields as follows:
%\begin{equation}
\begin{align}
\begin{split}
\vspace{-1em}
\notag
\label{eqn:query}
Query:= \langle Q_{ID}, A_{ID}, Sensors_{1 \to s}, \pi_{s_{Yes_{1}}}, \pi_{s_{Yes_{2}}}, \pi_{s_{No}}, \pi_1, \pi_2, \pi_3, \\ N, epoch, T_{start}, T_{end}, Version \rangle
\end{split}
\end{align}
%\end{equation}

Each query is uniquely identified by the query $Q_{ID}$ and analyst $A_{ID}$. The query is formulated as an $L$ bit vector over the IoT sensors.

$Sensors_{1 \to s}$ denotes the $S$ sensors to be monitored. Upon querying each sensor, the corresponding sensor value is then matched against the formulated query indexes. Each data owner's answer is in the form of a `1' or `0' per index, depending on whether or not the answer falls within that range.  Different ranges should not overlap.

$\pi_{s_{Yes_{1}}}$, $\pi_{s_{Yes_{2}}}$, and $\pi_{s_{No}}$ is the i.i.d. random sampling probability used to determine if a particular data owner of the $Yes$ and $No$ population should participate or not, respectively. $\pi_1$, $\pi_2$, $\pi_3$ denote the two coin toss probabilities coming up heads and are used privatize each data owner's response. The population of $Yes$ uses $\pi_1$ and $\pi_2$ where $\pi_1$ controls the truthful response and $\pi_2$ provides plausible deniability. The $No$ population data owners flips the coin $\pi_3$ to answer truthfully. The analyst requests a certain utility (expressed by the coin toss parameters) and the data owners may refuse if deemed risky.

$N$ defines the database size (i.e., the number of rows).

$epoch$ denotes the collection interval of the query, i.e., how often the query needs to be executed and responded by data owner. $T_{start}$ denotes the query start time and $T_{end}$ denotes the query end time, i.e., when answers to the query will no longer be accepted. The start time can be used when the query parameters are to be updated.

$Version$ defines the version number of the query parameters.

~ \\
\noindent \textbf{Query Update.} The aggregators can update the query between epochs (i.e., by setting a suitable $T_{start}$ time). Reasons might include increasing the database size $N$ to accommodate more data owners or to adjust the coin toss parameters to adjust the accuracy for the time of day (e.g., rush hour versus late night).

~ \\
\noindent \textbf{Query Audit.} The data owner's device audits~\cite{DBLP:journals/jcss/KleinbergPR03,DBLP:journals/csur/AdamW89,DBLP:journals/tse/ChinO82} and logs all the queries received from analysts and discards any query if its privacy cost $\epsilon$ (computed based on the query's $\pi_1$ and $\pi_2$) exceeds a certain configurable threshold.  For example, if location is asked too frequently or with too fine a granularity.The data owner is also able to restrict query execution based on a personal sensor blacklist. Analyst reputation may also be used to blacklist certain analyst queries from being executed.


==> setup.tex <==
\newtheoremstyle{mytheoremstyle}%                % Name
  {}%                                     % Space above
  {}%                                     % Space below
  {\itshape}%                             % Body font
  {}%                                     % Indent amount
  {\bfseries}%                            % Theorem head font
  {.}%                                    % Punctuation after theorem head
  { }%                                    % Space after theorem head, ' ', or \newline
  {}%                                     % Theorem head spec (can be left empty, meaning `normal')

%\theoremstyle{mytheoremstyle}
%\newtheorem{proposition}{Proposition}

%\newtheorem{definition}{Definition}
%\newtheorem{notation}{Notation}
%\newtheorem{lemma}{Lemma}
%\newtheorem{note}{Note}



==> systemmodel.tex <==
\subsection{System Model}

In prior systems only the data owners with the attribute matching the query privately respond. In our system model, all data owners in the population participate thereby increasing the privacy set (e.g., everyone in New York City replies as if they are at the Statue of Liberty). 

We now describe the system model. The system proceeds in epochs. Every epoch $t$ each data owner $i$ generates personal data (e.g. current location) on a device under their control (e.g., a smartphone or vehicle). There is a personal data stream $\mathbf{X}=$ $\{X_{t,i}\}$ where $0 \leq t < T$.

The data owner's personal data $X_{t,i}=\{x_{t,i,l}\}$ where $0 \leq l < L$ is a bit vector of length $L$, where $L$ is the number of queries (e.g., number of locations to monitor). While simple, binary classification can be extended to real-valued functions~\cite{DBLP:journals/jmlr/BshoutyF02}.

Next, each data owner generates a privatized (possibly randomized) view given their personal data $\mathbf{Z}=$ $\{Z_{t,i}|X_{t,i}\}$ where $0 \leq t < T$. Each entry $Z_{t,i}$ is a random variable in $t$, and is independently distributed across each $i$ entry though not identically distributed.

The contributions from data owners at epoch $t$ are aggregated to learn statistics about the population. We model the privatized data collected at each epoch as a statistical database as a vector $\mathbf{Z_t}=(Z_{t,1},...,Z_{t,i})$ where each entry $i$ has been contributed by a data owner. Each $i$ row is protected due to the cryptographic private write and the aggregator does not know which data owner wrote each $i$ entry as defined in ~\S\ref{def:privatewrite}.

Our learning domains are those within the Statistical Query (SQ) learning model~\cite{DBLP:conf/stoc/Kearns93}, whereby a binary value of a label may have noise added to it. We consider the class of all SQ learning algorithms for which efficient noise-tolerant algorithms exist. Essentially, we are interested in smooth functions whereby data perturbation only affects the output slightly.

The data $Z_{t,i}$ is privately released in response to a Statistical Query. Each data owner receives and processes a response to the local query $Q(Z_{t,i}~|~X_{t,i})$. The (exact) answer $a_q$ to a query $q$ at epoch $t$ is the sum of the data from all owners that contain the attribute being measured $a_q = \sum\nolimits_{i \in q} x_{t,i,q}$ (e.g., how many people are at a particular location).

%It should be noted that we adjust the definition of the population that responds to the counting query in order to satisfy \projecttitle privacy. That is, as opposed to prior systems whereby only the data owners with the attribute matching the query privately respond, in \projecttitle all data owners in the population participate thereby increasing the privacy set (e.g., everyone in London replies if they are at Buckingham Palace). That is, the (randomized) answer $a_q$ is the sum of all data owners in the population $a_q = \sum\nolimits_{i \in n} x_{t,i,q}$. In~\S\ref{sec:evaluation} we show that following this approach we still achieve high utility by subtracting the added privacy noise. 

